Does On-Policy Distillation Need to Complete Every Rollout?

On-policy distillation (OPD) transfers teacher knowledge to a student through feedback on student-generated rollouts, but generating complete rollouts and computing per-token teacher feedback are computationally expensive. Existing truncation methods save computation by stopping rollouts early. However, they do not compensate for truncated token gradients, which biases the gradient estimates and changes Vanilla OPD's original training objective. Furthermore, their truncation decisions rely on assumptions about supervision quality or criteria that may not generalize across settings. We introduce Stochastic Truncated On-Policy Distillation (STOPD), which accelerates OPD by randomly truncating student rollouts and correcting the resulting sampling bias with blockwise inverse-probability weighting (IPW). At each training step, we sample a stopping position for each rollout before generation and let the student generate until that position or natural termination. We obtain teacher feedback on every generated token and use blockwise IPW to compensate for the lower probability of retaining later tokens while controlling the weights. We prove that this weighting preserves Vanilla OPD's gradient sum in expectation and derive one-step update-error bounds for SGD, Adam, and Muon. We evaluate STOPD across multiple teacher-student model pairs, task domains, and optimizers. STOPD reduces generated tokens by 25-48% while maintaining accuracy comparable to Vanilla OPD, achieving 1.3-2.2x training speedups.

==> figs/tab_blockwidth.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{rrrcccccc}
\toprule
 & & & & \multicolumn{5}{c}{\textbf{Accuracy (\%) at step}}\\
\cmidrule(lr){5-9}
\textbf{\boldmath$K$} & \textbf{\boldmath$L/K$} & \textbf{Saved (\%)} & \textbf{Pred.\ SD} & \textbf{50} & \textbf{100} & \textbf{150} & \textbf{200} & \textbf{250}\\
\midrule
\multicolumn{2}{l}{Vanilla} & -- & --  & 24.1 & 26.9 & 28.5 & 28.1 & 30.1\\
32 & 512 & 34.6 & 0.99 & 24.1 & 27.1 & 28.2 & 29.2 & 29.8\\
128 & 128 & 34.3 & 0.98 & 24.4 & 27.5 & 29.0 & 27.9 & 29.4\\
512 & 32 & 33.1 & 0.93 & 24.1 & 27.7 & 28.8 & 28.7 & 29.7\\
2048 & 8 & 28.6 & 0.81 & 23.7 & 26.9 & 28.4 & 28.5 & 30.0\\
\bottomrule
\end{tabular}


==> figs/tab_dynamics.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{llrrrrr}
\toprule
 & & \multicolumn{3}{c}{\textbf{Mean}} & \multicolumn{2}{c}{\textbf{Jitter (\%)}}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
\textbf{Setting} & \textbf{Method} & \textbf{Entropy} & \textbf{Loss} & \textbf{Grad norm} & \textbf{Loss} & \textbf{Grad norm}\\
\midrule
\multicolumn{7}{l}{\textit{Main results: Qwen3-1.7B-Base $\leftarrow$ Qwen3-4B-Instruct-2507}}\\
\multirow{3}{*}{Math} & Vanilla & 0.315 & 0.413 & 0.90 & 1.7 & 3.4\\
 & \method{} & 0.348 & 0.419 & 1.08 & 7.2 & 9.0\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{4.3$\times$} & \textcolor{cornellred}{2.7$\times$}\\
\midrule
\multirow{3}{*}{Code} & Vanilla & 0.380 & 0.353 & 0.90 & 1.2 & 2.9\\
 & \method{} & 0.453 & 0.356 & 1.27 & 9.4 & 13.0\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.4$\times$} & \textcolor{cornellred}{7.7$\times$} & \textcolor{cornellred}{4.6$\times$}\\
\midrule
\multirow{3}{*}{Instruction following} & Vanilla & 1.018 & 0.630 & 2.79 & 5.0 & 6.8\\
 & \method{} & 1.065 & 0.643 & 3.05 & 13.2 & 14.4\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{2.7$\times$} & \textcolor{cornellred}{2.1$\times$}\\
\midrule
\multicolumn{7}{l}{\textit{Scaling: mathematics, Qwen3-30B-A3B-Instruct-2507 teacher}}\\
\multirow{3}{*}{Qwen3-4B-Base} & Vanilla & 0.319 & 0.268 & 0.54 & 1.5 & 6.3\\
 & \method{} & 0.333 & 0.272 & 0.67 & 7.2 & 12.1\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{4.9$\times$} & \textcolor{cornellred}{2.0$\times$}\\
\midrule
\multirow{3}{*}{Qwen3-8B-Base} & Vanilla & 0.312 & 0.250 & 0.52 & 1.6 & 5.2\\
 & \method{} & 0.322 & 0.254 & 0.64 & 7.8 & 10.4\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{5.0$\times$} & \textcolor{cornellred}{2.0$\times$}\\
\bottomrule
\end{tabular}


==> figs/tab_dynamics_optim.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{llrrrrr}
\toprule
 & & \multicolumn{3}{c}{\textbf{Mean}} & \multicolumn{2}{c}{\textbf{Jitter (\%)}}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
\textbf{Optimizer} & \textbf{Method} & \textbf{Entropy} & \textbf{Loss} & \textbf{Grad norm} & \textbf{Loss} & \textbf{Grad norm}\\
\midrule
\multirow{3}{*}{AdamW} & Vanilla & 0.316 & 0.413 & 0.89 & 1.5 & 3.2\\
 & \method{} & 0.348 & 0.418 & 1.07 & 7.5 & 8.1\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{5.1$\times$} & \textcolor{cornellred}{2.6$\times$}\\
\midrule
\multirow{3}{*}{SGD} & Vanilla & 0.209 & 0.335 & 1.02 & 2.4 & 2.7\\
 & \method{} & 0.272 & 0.338 & 1.13 & 9.5 & 10.9\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.3$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{4.0$\times$} & \textcolor{cornellred}{4.1$\times$}\\
\midrule
\multirow{3}{*}{Muon} & Vanilla & 0.271 & 0.370 & 0.91 & 2.0 & 3.1\\
 & \method{} & 0.307 & 0.373 & 1.06 & 7.6 & 9.5\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{3.8$\times$} & \textcolor{cornellred}{3.0$\times$}\\
\bottomrule
\end{tabular}


==> figs/tab_esr.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{3}{c}{\textbf{Training, steps 26--250}} & \multicolumn{3}{c}{\textbf{Evaluation at step 250}}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
\textbf{Method} & \textbf{Tokens} & \textbf{Time/step (s)} & \textbf{Time (h)} & \textbf{Accuracy (\%)} & \textbf{Length} & \textbf{Truncated (\%)}\\
\midrule
Vanilla & 9{,}516 & 941 & 58.8 & 30.1 & 10{,}685 & 19.1\\
\method{} & 6{,}255 & 513 & 32.1 & 29.4 & 11{,}414 & 22.0\\
ESR & 100 & 20 & 1.3 & 23.5 & 19{,}155 & 57.1\\
\bottomrule
\end{tabular}


==> figs/tab_optim.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{llcccccrr}
\toprule
 &  & \multicolumn{5}{c}{\textbf{Accuracy (\%) at step}} & & \\
\cmidrule(lr){3-7}
\textbf{Optimizer} & \textbf{Method} & \textbf{50} & \textbf{100} & \textbf{150} & \textbf{200} & \textbf{250} & \textbf{Tokens} & \textbf{Min/step}\\
\midrule
\multirow{3}{*}{SGD ($5\times10^{-4}$)} & Vanilla & 24.7 & 25.9 & 25.0 & 24.6 & 25.6 & 9{,}351 & 17.5\\
 & \method{} & 24.0 & 25.0 & 25.3 & 25.0 & 25.5 & 5{,}509 & 8.2\\
 & \textcolor{cornellred}{\textit{Speedup}} &  &  &  &  &  & \textcolor{cornellred}{1.7$\times$} & \textcolor{cornellred}{\textbf{2.1$\times$}}\\
\midrule
\multirow{3}{*}{Muon ($5\times10^{-6}$)} & Vanilla & 23.6 & 25.3 & 26.3 & 28.2 & 29.6 & 10{,}014 & 17.1\\
 & \method{} & 24.2 & 25.2 & 25.5 & 28.2 & 30.0 & 6{,}248 & 9.1\\
 & \textcolor{cornellred}{\textit{Speedup}} &  &  &  &  &  & \textcolor{cornellred}{1.6$\times$} & \textcolor{cornellred}{\textbf{1.9$\times$}}\\
\bottomrule
\end{tabular}


==> figs/tab_results_batch.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{lccccccccccc}
\toprule
 & & \multicolumn{10}{c}{\textbf{IFEval (\%) at step}}\\
\cmidrule(lr){3-12}
\textbf{Method} & \textbf{Base} & \textbf{5} & \textbf{10} & \textbf{15} & \textbf{20} & \textbf{25} & \textbf{30} & \textbf{35} & \textbf{40} & \textbf{45} & \textbf{50}\\
\midrule
Vanilla & \multirow{2}{*}{15.6} & \multirow{2}{*}{16.2$_{\pm0.1}$} & 17.4$_{\pm0.2}$ & 18.0$_{\pm0.1}$ & 25.3$_{\pm0.8}$ & 29.4$_{\pm0.5}$ & 30.5$_{\pm0.2}$ & 32.9$_{\pm0.5}$ & 35.9$_{\pm0.6}$ & 38.5$_{\pm0.8}$ & 40.5$_{\pm0.7}$\\
\method{} & & & 17.4$_{\pm0.2}$ & 17.5$_{\pm0.5}$ & 25.3$_{\pm0.4}$ & 28.6$_{\pm0.3}$ & 30.1$_{\pm0.2}$ & 32.8$_{\pm0.4}$ & 35.4$_{\pm0.5}$ & 37.8$_{\pm0.7}$ & 40.0$_{\pm0.4}$\\
\bottomrule
\end{tabular}


==> figs/tab_results_noreweight.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{lccccccccccc}
\toprule
 & & \multicolumn{10}{c}{\textbf{Accuracy (\%) at step}}\\
\cmidrule(lr){3-12}
\textbf{Method} & \textbf{Base} & \textbf{25} & \textbf{50} & \textbf{75} & \textbf{100} & \textbf{125} & \textbf{150} & \textbf{175} & \textbf{200} & \textbf{225} & \textbf{250}\\
\midrule
\multicolumn{12}{l}{\textit{Mathematics: Qwen3-1.7B-Base $\leftarrow$ Qwen3-4B-Instruct-2507}}\\
Vanilla & \multirow{3}{*}{11.7} & \multirow{3}{*}{23.4$_{\pm0.8}$} & 24.1$_{\pm0.0}$ & 27.9$_{\pm0.7}$ & 26.9$_{\pm0.2}$ & 28.4$_{\pm0.6}$ & 28.5$_{\pm0.7}$ & 29.3$_{\pm0.4}$ & 28.1$_{\pm1.8}$ & 30.0$_{\pm0.4}$ & 30.1$_{\pm0.5}$\\
\method{} &  &  & 24.4$_{\pm0.9}$ & 27.3$_{\pm0.7}$ & 27.5$_{\pm0.5}$ & 27.7$_{\pm0.6}$ & 29.0$_{\pm0.5}$ & 29.1$_{\pm0.1}$ & 27.9$_{\pm1.4}$ & 28.5$_{\pm0.6}$ & 29.4$_{\pm0.6}$\\
\method{}, $w_t=1$ &  &  & 23.8$_{\pm0.2}$ & 27.4$_{\pm0.1}$ & 26.9$_{\pm0.4}$ & 27.7$_{\pm0.4}$ & 27.9$_{\pm0.5}$ & 29.2$_{\pm0.6}$ & 29.0$_{\pm0.5}$ & 29.6$_{\pm0.3}$ & 29.1$_{\pm0.3}$\\
\midrule
\multicolumn{12}{l}{\textit{Mathematics: Qwen3-4B-Base $\leftarrow$ Qwen3-30B-A3B-Instruct-2507}}\\
Vanilla & \multirow{3}{*}{15.2} & \multirow{3}{*}{34.9$_{\pm0.8}$} & 34.7$_{\pm0.7}$ & 41.1$_{\pm0.7}$ & 44.0$_{\pm0.6}$ & 44.2$_{\pm0.2}$ & 45.0$_{\pm0.5}$ & 45.0$_{\pm0.4}$ & 46.2$_{\pm0.9}$ & 46.3$_{\pm0.3}$ & 46.2$_{\pm0.2}$\\
\method{} &  &  & 34.7$_{\pm0.6}$ & 40.1$_{\pm0.6}$ & 43.5$_{\pm0.2}$ & 43.7$_{\pm0.3}$ & 44.9$_{\pm0.7}$ & 44.9$_{\pm0.5}$ & 45.5$_{\pm0.6}$ & 46.3$_{\pm0.7}$ & 45.3$_{\pm0.4}$\\
\method{}, $w_t=1$ &  &  & 33.9$_{\pm0.7}$ & 38.8$_{\pm0.2}$ & 41.8$_{\pm0.9}$ & 43.7$_{\pm1.0}$ & 44.7$_{\pm0.8}$ & 45.1$_{\pm1.1}$ & 45.3$_{\pm0.3}$ & 45.7$_{\pm0.7}$ & 45.9$_{\pm0.2}$\\
\bottomrule
\end{tabular}


==> figs/tab_results_tir.tex <==
% Generated from archived TIR data; mean +/- sample SD across three seeds.
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{\textbf{With interpreter}} & \multicolumn{2}{c}{\textbf{Without interpreter}}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Step} & \textbf{Vanilla} & \textbf{\method{}} & \textbf{Vanilla} & \textbf{\method{}}\\
\midrule
Initial & \multicolumn{2}{c}{31.1} & \multicolumn{2}{c}{42.4}\\
25 & 53.8$_{\pm0.6}$ & 53.8$_{\pm0.6}$ & 52.8$_{\pm0.8}$ & 52.8$_{\pm0.8}$\\
50 & 56.5$_{\pm0.6}$ & 57.0$_{\pm0.7}$ & 58.4$_{\pm0.8}$ & 58.5$_{\pm0.6}$\\
75 & 57.9$_{\pm0.4}$ & 58.5$_{\pm0.4}$ & -- & --\\
100 & 59.5$_{\pm0.6}$ & 58.4$_{\pm0.4}$ & 58.5$_{\pm0.4}$ & 59.0$_{\pm0.3}$\\
125 & 58.8$_{\pm0.4}$ & 59.2$_{\pm0.6}$ & -- & --\\
150 & 59.4$_{\pm0.7}$ & 59.6$_{\pm0.5}$ & 57.6$_{\pm0.5}$ & 58.0$_{\pm0.4}$\\
175 & 59.0$_{\pm0.5}$ & 59.2$_{\pm0.2}$ & -- & --\\
200 & 60.0$_{\pm0.6}$ & 59.2$_{\pm0.5}$ & 58.5$_{\pm0.5}$ & 59.0$_{\pm0.5}$\\
\midrule
Teacher & \multicolumn{2}{c}{60.0} & \multicolumn{2}{c}{65.3}\\
\bottomrule
\end{tabular}


==> figs/tab_time_batch.tex <==
% Generated by figs/make_figures.py; do not edit.
\begin{tabular}{llrrrrrr}
\toprule
\multicolumn{4}{l}{\textit{Qwen3-1.7B-Base $\leftarrow$ Qwen3-4B-Instruct-2507}} & \multicolumn{4}{c}{\textbf{Time per step (s)}}\\
\cmidrule(lr){5-8}
\textbf{Batch size} & \textbf{Method} & \textbf{Tokens} & \textbf{k tok/s} & \textbf{Generation} & \textbf{Update} & \textbf{Other} & \textbf{Total}\\
\midrule
\multirow{3}{*}{256} & Vanilla & 710 & 3.8 & 54 & 36 & 14 & 104\\
 & \method{} & 533 & 3.8 & 39 & 29 & 12 & 80\\
 & \textcolor{cornellred}{\textit{Speedup}} & \textcolor{cornellred}{1.3$\times$} & \textcolor{cornellred}{1.0$\times$} & \textcolor{cornellred}{1.4$\times$} & \textcolor{cornellred}{1.2$\times$} & \textcolor{cornellred}{1.1$\times$} & \textcolor{cornellred}{\textbf{1.3$\times$}}\\
\midrule
\multirow{3}{*}{2048} & Vanilla & 820 & 5.5 & 308 & 232 & 92 & 632\\
 & \method{} & 595 & 5.1 & 240 & 171 & 66 & 478\\
 & \textcolor{cornellred}{\textit{Speedup}} & \textcolor{cornellred}{1.4$\times$} & \textcolor{cornellred}{0.9$\times$} & \textcolor{cornellred}{1.3$\times$} & \textcolor{cornellred}{1.4$\times$} & \textcolor{cornellred}{1.4$\times$} & \textcolor{cornellred}{\textbf{1.3$\times$}}\\
\bottomrule
\end{tabular}


==> figs/tab_time_tir.tex <==
% Student tokens exclude tool observations. Other includes old-log-probability computation, checkpoint writing, and weight synchronization.
\begin{tabular}{llrrrrrr}
\toprule
\multicolumn{4}{l}{\textit{Qwen3-4B $\leftarrow$ Qwen3-30B-A3B-Instruct-2507}} & \multicolumn{4}{c}{\textbf{Time per step (s)}}\\
\cmidrule(lr){5-8}
\textbf{Domain} & \textbf{Method} & \textbf{Tokens} & \textbf{k tok/s} & \textbf{Generation} & \textbf{Update} & \textbf{Other} & \textbf{Total}\\
\midrule
TIR & Vanilla & 7{,}184 & 1.64 & 1118 & 828 & 216 & 2163\\
 & \method{} & 5{,}193 & 1.94 & 685 & 568 & 151 & 1404\\
 & \textcolor{cornellred}{\textit{Ratio}} & \textcolor{cornellred}{1.38$\times$} & \textcolor{cornellred}{1.18$\times$} & \textcolor{cornellred}{1.63$\times$} & \textcolor{cornellred}{1.46$\times$} & \textcolor{cornellred}{1.43$\times$} & \textcolor{cornellred}{1.54$\times$}\\
\bottomrule
\end{tabular}

